hMAC: Enabling Hybrid TDMA/CSMA on IEEE 802.11 Hardware

We present our current work-in-progress on the design and implementation of a hybrid TDMA/CSMA medium access architecture, hereafter referred to as hMAC, which can be used on top of commercial IEEE 802.11 off-the-shelf hardware. The software only solution is based on the popular Linux ATH9K softMAC driver and hence can be used with standard Linux systems using Atheros based wireless network devices. The proposed hMAC exploits the standard 802.11 power saving functionality present in the ATH9K device driver to enable control of the software packet queues. This allows the assignment of TDMA time slots on wireless link and traffic class basis. While the solution is placed only in the device driver, the CSMA/CA functionality on hardware level is still active. This enables inter-working with standard unmodified 802.11 devices. We tested our prototypical hMAC implementation in a small test-bed. Therefore, we implemented a centralized interference management scheme in which pairs of links suffering from a hidden node problem are assigned to TDMA time slots on a per-link basis. To show the benefits of the proposed hMAC approach we compared the results with standard 802.11 DCF and classical, i.e. per-node, TDMA. Finally, to enable collaboration with the research community, the hMAC source code is provided as open-source.

==> packages/config.tex <==
%!TEX root = ../techreport.tex

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{tabularx}
\usepackage{multicol}
\usepackage{graphicx}

\usepackage{tikz}
\usepackage{lipsum}

\usepackage[headsepline,plainheadsepline,footsepline,plainfootsepline]{scrpage2}


\usepackage{mathptmx}
\usepackage[scaled=.92]{helvet}
\usepackage{courier}

% ================================================================
% FIXME package setup
% ================================================================
\usepackage[multiuser,nomargin,marginclue,footnote]{fixme}
% use different colors for fixme levels
\fxusetheme{color}
\fxsetup{targetlayout=colorcb}
% define authors for fixme
% \FXRegisterAuthor{commnad prefix}{environment prefix}{tag}
\FXRegisterAuthor{awo}{anawo}{AWO}
\FXRegisterAuthor{mc}{anmc}{Mikolaj}
% Usage example \mcfatal{Has to be fixed ASAP}
% Usage example \mcerror{Problem}
% Usage example \mcwarning{Possible problem}
% Usage example \mcnote{Comment}
% fixme mode
% change 'draft' to 'final' for final version
\fxsetup{status=draft}


% ================================================================
% Page Style
% ================================================================

\usepackage{geometry}
\geometry{a4paper, inner=30mm, outer=25mm, top=40mm, bottom=42mm}


\clearscrheadfoot

\ihead[\Large {\scshape TKN Technical Report Series / Technische Universität Berlin }]{\Large {\scshape TU Berlin }}

\ifoot[{\tiny \begin{minipage}{4.0cm}Copyright at Technische Universität Berlin.\newline All Rights reserved.\end{minipage}}]{{\tiny \begin{minipage}{4.0cm}Copyright at Technische Universität Berlin.\newline All Rights reserved.\end{minipage}}}
\cfoot[\scriptsize \trnumber]{\scriptsize \trnumber}
\ofoot[Page \pagemark]{Page \pagemark}

\pagestyle{scrheadings}

\addtokomafont{pagefoot}{\normalfont}



\bibliographystyle{plain}

